Backward Raman Amplification in the Long-wavelength Infrared

The wealth of work in backward Raman amplification in plasma has focused on the extreme intensity limit, however backward Raman amplification may also provide an effective and practical mechanism for generating intense, broad bandwidth, long-wavelength infrared radiation (LWIR). An electromagnetic simulation coupled with a relativistic cold fluid plasma model is used to demonstrate the generation of picosecond pulses at a wavelength of 10 microns with terawatt powers through backward Raman amplification. The effects of collisional damping, Landau damping, pump depletion, and wave breaking are examined, as well as the resulting design considerations for a LWIR Raman amplifier.

==> makefile <==
# set latexfile to the name of the main file without the .tex
latexfile = main
bibtexfile = main
TEX = latex

# Determine OS
UNAME := $(shell uname -s)
ifeq ($(UNAME),Darwin)
	OS := Apple
endif
ifeq ($(UNAME),Linux)
	OS := Linux
endif

# reruns latex if needed.  to get rid of this capability, delete the
# three lines after the rule.  Delete .bbl dependency if not using
# BibTeX references.
# idea from http://ctan.unsw.edu.au/help/uk-tex-faq/Makefile

# make sure the all git calls happen before latex is run
$(latexfile).dvi : $(latexfile).tex git  uncommitted commitdate bib
	while ($(TEX) $(latexfile) ;  grep -q "Rerun to get cross" $(latexfile).log ) do true ;  done
	rm currentcommit.tmp   # remove next three lines if not using git repo  
	rm uncommitted-files.tmp 
	rm commit-date.tmp

git :
	git show --summary --format="%h" > currentcommit.tmp


uncommitted :
	git status --short | wc -l | tr -d " " > uncommitted-files.tmp


commitdate:
	git show --summary --format="%ad" --date=local > commit-date.tmp


$(latexfile).pdf : $(latexfile).ps
	ps2pdf $(latexfile).ps $(latexfile).pdf


pdf : $(latexfile).pdf


$(latexfile).ps : $(latexfile).dvi
	dvips $(latexfile)


ps : $(latexfile).ps 

# make can't know all the sourcefiles.  some file may not have
# sourcefiles, e.g. eps's taken from other documents. 
$(latexfile).tar.gz :  $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $^

tarball: $(latexfile).tar.gz

bib: 
	latex $(latexfile).tex
	bibtex $(bibtexfile).aux
	bibtex $(bibtexfile).aux

# use make diff old=15c6254727411678 new=15c6254727411678
#     make diff old=15c6254727411678 (head is assumed)
# 
diff: 
	git latexdiff --latex --bibtex --main $(latexfile).tex $(old) $(new)

view: 
ifeq ($(OS),Apple)
	open $(latexfile).pdf
endif
ifeq ($(OS),Linux)
	evince $(latexfile).pdf &
endif

clean:
	rm -f *.log *.aux *.blg *.bbl 

purge: clean
	rm -f *.pdf *.ps *.dvi pack.zip

# zips the tex and bib files
#  Use he following to find used figure names
#       sed -n -e 's/^[[:space:]]*\\includegraphics.*{//p' $(latexfile).tex | sed -e 's/}.*/.eps/' 
pack:
	mv main.bib dirty.bib;
	# remove personal annotations
	sed -e 's/annotate={.*}/annotate={}/' dirty.bib > main.bib
	zip pack.zip $(latexfile).tex $(bibtexfile).bib 
	# Replace clean bib file with the one with annotations
	mv dirty.bib main.bib
	# Pack up .bbl file for arXiv submission
	zip pack.zip main.bbl
	# pack up the figures
	zip pack.zip ./fig/time-series.eps
	zip pack.zip ./fig/contour.eps
	zip pack.zip ./fig/contour800nm.eps
	zip pack.zip ./fig/figure3.eps
	zip pack.zip ./fig/seed_duration_scan.eps
	zip pack.zip ./fig/2d-sim.eps
	zip pack.zip ./fig/ei-collision-time.eps
	zip pack.zip ./fig/en-collision-time.eps
	# Pack up the makefile
	zip pack.zip makefile

